DoGR: Disaggregated Gaussian Regression for Reproducible Analysis of Heterogeneous Data

Quantitative analysis of large-scale data is often complicated by the presence of diverse subgroups, which reduce the accuracy of inferences they make on held-out data. To address the challenge of heterogeneous data analysis, we introduce DoGR, a method that discovers latent confounders by simultaneously partitioning the data into overlapping clusters (disaggregation) and modeling the behavior within them (regression). When applied to real-world data, our method discovers meaningful clusters and their characteristic behaviors, thus giving insight into group differences and their impact on the outcome of interest. By accounting for latent confounders, our framework facilitates exploratory analysis of noisy, heterogeneous data and can be used to learn predictive models that better generalize to new data. We provide the code to enable others to use DoGR within their data analytic workflows.

==> problem.tex <==
\section{Problem Formulation}
Let $\mathcal{D} = {d_1, d_2, d_3, ..., d_n | d_i = (x_i, y_i) \in \mathcal{R}^p \times R}$ be a set of $n$ observations described by a real-valued outcome variable $y$, and $p$ real-values independent variables $x_1, x_2, ..., x_p$. Each observation $d_i$ is describe by pair of $(x_i, y_i)$ where $x_i$ is a vector of independent variables $[x_{i, 1}, x_{i, 2}, ..., x_{i, p}]$ and $y_i$ is outcome variable of observation $i$. Our goal is to capture the relationship of each independent variable and outcome variable as \textit{realistic} as possible. For example, using traditional \textit{Multivariate Linear Regression (MLR)}, the parameters $\beta_0, \beta_1, ..., \beta_p$ can be find such that the residual of model $y = \beta_0 + \beta_1 x_1 + \beta_2 x_2 + ... + \beta_p x_p$ over all observations is minimized. However, the learned parameters in \textit{MLR} model is not \textit{realistic}. Here \textit{realistic} is related to cases where Simpson's Paradox happens.

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.48\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{Figures/example_equal_size.pdf}
%         \caption{Balanced components}\label{fig:explain-balanced}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.48\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{Figures/example_unbalanced.pdf}
%         \caption{Unbalanced components}\label{fig:explain-unbalanced}
%     \end{subfigure}
     
%     \caption{Red line is regression line of Multivariate Linear Regression. Dashed green lines are regression lines of components of our model, and solid green line is regression line of our model. When number of data points in all components are balanced, then MLR has positive coefficient for $y$ in terms of $x_1$. However, the coefficient is zero in unbalanced data. The coefficient would be even negative for heavier unbalanced data. But the coefficient of \ourMethod components remain the same. \label{fig:explain}}
% \end{figure}

 Figure \ref{fig:explain}, represents a synthetic example where \textit{MLR} model is equal to $y = 56.41 + 0.61  x_1$, which suggests a positive correlation between $x_1$ and $y$. However, we can see that the correlation between $x_1$ and $y$ is negative in each of three components ($y = c - x_1$, where $c$ is cluster's intercept, $201, 302, 393$). Thus, the MLR model is \textit{misleading} in capturing the relationship between $x_1$ and $y$. In this case, data has three different regression line for each cluster (dashed green lines). Combining these three clusters regression line, we can have a better regression model. More precisely, the Root Mean Squared Error (RMSE) for \textit{MLR} model is $33.07$ and Mean Absolute Error (MAE) is $26.50$, while both measure are smaller for our model: RMSE = $31.38$ and MAE = $24.85$. \nazanin{remove this and update text since it is in related work section} There are bunch of papers who showed the accuracy of regression line is much more higher in cluster-wise linear regression \cite{spath, manwani2015, desarbo1988maximum, sung2004, ghahramani1994, silva2017, silva2018, calderon2018}. Even tough our method has novelty in compare with literature, the focus of this paper is much more on using cluster-wise regression algorithm on finding surprising patterns. We will get advantage from comparing results of semi-supervised regression methods and supervised regression methods to find surprising patterns in data. 
 
 Let's call $\mathcal{M}$ a cluster-wise regression model with $k$ clusters. For each cluster $i$, we have a regression coefficient $\beta_i \in \mathcal{R}^{p+1}$. The regression value of cluster $i$ would be $\hat{y}^{(i)} = \beta_{i, 0} + \beta_{i, 1} x_{1} + \beta_{i, 2} x_{2} + ... + \beta_{i, p} x_{p}$. Model $\mathcal{M}$ is a regression model, so the regression value of $y$ would be a function of regression value of all components: $\hat{y} = f(\hat{y}^{(1)}, \hat{y}^{(2)}, ..., \hat{y}^{(k)})$. In this case, model $\mathcal{M}$ would be a good regression model if (1) it leverage \textbf{Simpson's Paradox} to help data scientist and (2) it predicts value of $y$ accurately. We can define error of regression line as $e = |y - \hat{y}|$
 

==> table.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cccc}
        Method & Hyperparameters & MAE (+std) & RMSE (+std) \\
        \toprule 
        \multicolumn{4}{c}{Concrete} \\ 
        \midrule
        MLR &  & $0.10 \pm 0.0065$ & $0.13 \pm 0.0076$ \\
        CLR & K : 1 & $0.10 \pm 0.0065$ & $0.13 \pm 0.0076$\\ 
        KPLANE & K : 4 $\gamma$ : 10 & $0.088 \pm 0.0053$ & $0.11 \pm 0.0072$ \\
        WCLR & K : 4 $\alpha$ : 0.1 & $0.078 \pm 0.0056$ & $0.10 \pm 0.0063$\\
        FWCLR & K : 3 $\alpha$ : 10 m : 1.1 & $0.076 \pm 0.0056$ & $0.10 \pm 0.0075$ \\
        GMR & K : 5 & $0.083 \pm 0.0064$ & $0.11 \pm 0.0100$ \\
        \bottomrule
        
        \multicolumn{4}{c}{Forestfires} \\ 
        \midrule
        MLR & & $0.02 \pm 0.0074$ & $0.043 \pm 0.042$\\
        CLR & K : 1 & $0.02 \pm 0.0074$ & $0.043 \pm 0.042$ \\ 
        KPLANE & K : 2 $\gamma$ : 0.1 & $0.017 \pm 0.0083$ & $0.042 \pm 0.043$ \\
        WCLR & K : 1 $\alpha$ : 0.001 & $0.02 \pm 0.0074$ & $0.043 \pm 0.042$\\
        FWCLR & K : 3 $\alpha$ : 100 m : 1.1 & $0.017 \pm 0.008$ & $0.042 \pm 0.043$\\
        GMR & K : 1 & $0.018 \pm 0.006$ & $0.044 \pm 0.038$ \\
        \bottomrule
        
        \multicolumn{4}{c}{WineQuality-Red} \\ 
        \midrule
        MLR & & $0.10 \pm 0.0051$ & $0.13 \pm 0.0079$ \\
        CLR & K : 1 & $0.10 \pm 0.0051$ & $0.13 \pm 0.0079$ \\ 
        KPLANE & K : 3 $\gamma$ : 100 & $0.10 \pm 0.0049$ & $0.13 \pm 0.0074$ \\
        WCLR & K : 3 $\alpha$ : 0.001 & $0.10 \pm 0.0049$ & $0.13 \pm 0.0072$\\
        FWCLR & K : 3 $\alpha$ : 0.01 m : 1.1 & $0.10 \pm 0.005$ & $0.13 \pm 0.0074$ \\
        GMR & K : 2 & $0.10 \pm 0.005$ & $0.13 \pm 0.0062$ \\
        \bottomrule
        
        \multicolumn{4}{c}{WineQuality-White} \\ 
        \midrule
        MLR & & $0.098 \pm 0.0021$ & $0.13 \pm 0.0036$ \\
        CLR & K : 1 & $0.098 \pm 0.0021$ & $0.13 \pm 0.0036$ \\ 
        KPLANE & K : 4 $\gamma$ : 100 & $0.095 \pm 0.0024$ & $0.12 \pm 0.0036$\\
        WCLR & K : 4 $\alpha$ : 0.001 & $0.094 \pm 0.0024$ & $0.12 \pm 0.0034$\\
        FWCLR & K : 4 $\alpha$ : 0.1 m : 1.1 & $0.094 \pm 0.0021$ & $0.12 \pm 0.0033$\\
        GMR & K : 5 & $0.092 \pm 0.0030$ & $0.12 \pm 0.0037$ \\
        \bottomrule
         
        \multicolumn{4}{c}{YachtHydrodynamics} \\ 
        \midrule
        MLR & & $0.12 \pm 0.01$ & $0.14 \pm 0.017$ \\
        CLR & K : 2 & $0.05 \pm 0.019$ & $0.087 \pm 0.028$ \\ 
        KPLANE & K : 2 $\gamma$ : 0.1 & $0.041 \pm 0.012$ & $0.07 \pm 0.023$ \\
        WCLR & K : 3 $\alpha$ : 100 & $0.016 \pm 0.004$ & $0.027 \pm 0.0077$ \\
        FWCLR & K : 3 $\alpha$ : 100 m : 1.1 & $0.017 \pm 0.0031$ & $0.027 \pm 0.0052$ \\
        GMR & K : 2 & $0.03 \pm 0.0065$ & $0.044 \pm 0.0095$\\
        \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
